Anomaly Detection in High Performance Computers: A Vicinity Perspective

In response to the demand for higher computational power, the number of computing nodes in high performance computers (HPC) increases rapidly. Exascale HPC systems are expected to arrive by 2020. With drastic increase in the number of HPC system components, it is expected to observe a sudden increase in the number of failures which, consequently, poses a threat to the continuous operation of the HPC systems. Detecting failures as early as possible and, ideally, predicting them, is a necessary step to avoid interruptions in HPC systems operation. Anomaly detection is a well-known general purpose approach for failure detection, in computing systems. The majority of existing methods are designed for specific architectures, require adjustments on the computing systems hardware and software, need excessive information, or pose a threat to users' and systems' privacy. This work proposes a node failure detection mechanism based on a vicinity-based statistical anomaly detection approach using passively collected and anonymized system log entries. Application of the proposed approach on system logs collected over 8 months indicates an anomaly detection precision between 62% to 81%.

==> data-source.tex <==
\section{Data Sources}
\label{sec:data-source}

System logs are the main source of information in this work.
Syslog daemons on each node collect the system log entries and forward them to a central log collector.
To maintain the neutrality of the results, the pre-configured syslog daemons (by Taurus manufacturer) were used without any changes.

In addition to syslog entries, three other sources of information were employed to increase the accuracy of final results: \emph{outages database}, \emph{service notifications}, and \emph{jobs status report}.
The outages database reports all system outages from the users perspective, the service notifications notify users of future scheduled maintenances and system-wide outages, and the job status reports indicate the final status of a job after its allocation.
\autoref{tab:data-sources} provides an overview of the four data sources which are used in this work.

\begin{table}[!t]
	\linespread{0.9}
	\fontsize{6.9pt}{10pt}\selectfont
	\caption{Data sources}
	\centering
	\begin{tabular}{l|l|l|l}
		\textbf{Data source} & \textbf{Data collection} & \textbf{Information} & \textbf{Granularity} \\
		\hline
		System logs & Automatic & Software and hawrdware & Component \\
		Outages database & Semi-automatic & Service availability & Entire system \\
		Service notifications & Manual & Service availability & Entire system \\
		Jobs status report & Automatic & Job completion status & Node \\

	\end{tabular}
	\label{tab:data-sources}
\end{table}

Preliminary analysis of the four data sources indicated certain gaps in the available data.
The gaps are mainly incurred due to the interruption of the data collection mechanisms.
Syslog entries as shown in \autoref{fig:syslog-overview} are covering the full period of one year from January to December 2017.
The jobs status report generated by Slurm is covering more than eight months from March to November 2017.
\autoref{fig:slurm-overview} illustrates the available jobs status report for the period of 28-02-2017 to 14-11-2017.
Service notifications and outages database as shown in \autoref{fig:service-overview} and \autoref{fig:manual-db-overview} provide information from a higher perspective and are available for the whole period of one year from January to December 2017.

According to the available information the focus in this study will be on the period of 01-03.2017 to 13-11-2017.
Lacking all data sources for a long continuous period of time is a known challenge in other similar studies \cite{Sayed2013}.

\begin{figure}
	\begin{center}
		\includegraphics[trim= 20 0 10 70, clip, width=.45\textwidth]{./Figure/{syslog-daily}.png}
		\caption{Collected system logs on all islands of Taurus for year 2017. Intervals of unavailability of syslog entries do not necessarily specify node outages.}
		\label{fig:syslog-overview}
	\end{center}
	\vspace{-0.2cm}
\end{figure}


\begin{figure}
	\begin{center}
		\includegraphics[trim= 20 0 10 70, clip, width=.45\textwidth]{./Figure/{slurm}.png}
		\caption{Slurm job status report on all islands of Taurus for year 2017. Intervals of unavailability of job reports do not necessarily specify node outages.}
		\label{fig:slurm-overview}
	\end{center}
	\vspace{-0.2cm}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[trim= 0 0 10 130, clip, width=.45\textwidth]{./Figure/{service}.png}
		\caption{Service notificatino on all islands of Taurus for year 2017.}
		\label{fig:service-overview}
	\end{center}
	\vspace{-0.2cm}
\end{figure}


\begin{figure}
	\begin{center}
		\includegraphics[trim= 0 0 10 110, clip, width=.45\textwidth]{./Figure/{manual-db}.png}
		\caption{Availability of Taurus in year 2017 from administrators perspective. Intervals of unknown availability do not necessarily specify the unavailability of services.}
		\label{fig:manual-db-overview}
	\end{center}
	\vspace{-0.2cm}
\end{figure}


==> failures.tex <==
\section{Identifying Regular Failures}
\label{sec:failures}

Node failures in computing systems can be divided into two categories according to their cause.
Some failures are occurring regularly during the normal operation of the system and are caused by internal factors such as software and hardware errors or racing conditions.
While others are occurring due to external causes such as power outage, unsuccessful maintenances, or human errors.
Analyzing the impact of external causes on node failures requires additional information which are not available.
Therefore, this work focuses on the first group of node failures which are \emph{regular failures} and caused by internal factors.
The first step to identify failures is detecting node outages and then distinguishing regular failures from those which may happen as a result of external factors such as maintenances, human errors, and so forth.

In this work, system logs are the main source of information.
Syslog entries are generated by individual remote nodes and sent to the central log collector which stores them for future analysis.
This passive log collection mechanism is chosen since it imposes no additional overhead on Taurus and is applicable to all HPC systems.
However, the failure identification process becomes more challenging.

Due to employment of the passive log collection mechanism, a node outage can be confidently detected only when a direct indication in form of a log entry is generated by the failing node and correctly received and stored by the central log collector, e.g. "Kernel panic - not syncing: Fatal Exception."
However, in many cases a node outage leaves no direct indication in system logs.
A workaround is to assume the absence of log entries for more than a certain period of time as an indication of a potential outage.
Nonetheless, this assumption is also not accurate.
For various reasons the flow of system log entries from computing nodes to the central log collector might be interrupted or delayed, which might be considered as an outage although the computing nodes are still functional.
Also, in many cases immediately after the occurrence of an outage, protection mechanisms recover the node.
In the both later scenarios, an active node probing approach might also fail in correct detection of all node outages.

Via analyzing Taurus system logs it has became experimentally evident that all nodes during a healthy boot, leave similar footprints in syslog entires.
If a node fails to generate the expected footprint at boot time, it is an indication of a faulty boot process and thus the node will be either automatically rebooted again or fails shortly afterwards.
The higher frequency of log generation at boot time in compare with the normal operation is another indicator of a boot event, which can be used to identify even a problematic boot process.

In this study for detecting node outages, first the nodes boot events are detected.
After detection of a boot event, syslog entries are tracked back until the last syslog entry before the boot event is being found.
The timestamp of last syslog entry before the boot event is considered as the point of outage.
Using the proposed method, all node outages will be identified.
The only exception is when a node fails and has no further successful boot process.
In such cases, comparing the timestamp of the last available syslog entry with the current time (in this study: $31$-$12$-$2017$ $23$:$59$:$59$) reveals the missing outages.
\autoref{fig:syslog-events} illustrates all detected outages on Taurus within the period of one year.

\begin{figure}
	\begin{center}
		\includegraphics[trim= 20 0 10 70, clip, width=.45\textwidth]{./Figure/{syslog-events}.png}
		\caption{Node outages detected via syslog analysis. Unexpected events (shown in red) indicate the absence of information in system logs which might be sign of potential crashes. Expected events indicate node outages which are planned due to maintenance or initiated via protection mechanisms.}
		\label{fig:syslog-events}
	\end{center}
	\vspace{-0.2cm}
\end{figure}

All outages detected via syslog analyzing are compared against the other three available data sources (\autoref{tab:data-sources}).
When a node outage is happened out of the scheduled maintenance period, and no job could be accomplished on that particular node at the time of the detected outage, the detected outage is a failure.
As \autoref{fig:slurm-failure} illustrates, it is common that certain jobs on a specific node fail although other jobs on the same node are accomplished simultaneously.
Also, when a node outage is indicated in the outages database, which monitors the availability of the HPC system from users perspective, it will be considered as a failure.
The workflow of failure detection in Taurus is shown in \autoref{fig:workflow}.

\begin{figure}
	\begin{center}
		\includegraphics[trim= 20 0 10 70, clip, width=.45\textwidth]{./Figure/{slurm-failure}.png}
		\caption{Slurm job status report on all islands of Taurus for year 2017. Intervals of unavailability of job reports do not necessarily specify node outages. The red dots indicate jobs which are failed due to a node failure.}
		\label{fig:slurm-failure}
	\end{center}
	\vspace{-0.2cm}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[trim= 60 0 60 0, clip, width=.45\textwidth]{./Figure/{flowchart}.pdf}
		\caption{Workflow of failure detection in Taurus via system logs. In case of having both contradicting results at once, the incident will not be considered as a failure.}
		\label{fig:workflow}
	\end{center}
	\vspace{-0.2cm}
\end{figure}



